Consistency Regularization Can Improve Robustness to Label Noise

Consistency regularization is a commonly-used technique for semi-supervised and self-supervised learning. It is an auxiliary objective function that encourages the prediction of the network to be similar in the vicinity of the observed training samples. Hendrycks et al. (2020) have recently shown such regularization naturally brings test-time robustness to corrupted data and helps with calibration. This paper empirically studies the relevance of consistency regularization for training-time robustness to noisy labels. First, we make two interesting and useful observations regarding the consistency of networks trained with the standard cross entropy loss on noisy datasets which are: (i) networks trained on noisy data have lower consistency than those trained on clean data, and(ii) the consistency reduces more significantly around noisy-labelled training data points than correctly-labelled ones. Then, we show that a simple loss function that encourages consistency improves the robustness of the models to label noise on both synthetic (CIFAR-10, CIFAR-100) and real-world (WebVision) noise as well as different noise rates and types and achieves state-of-the-art results.

==> 1_introduction.tex <==
\vspace{-0.4cm}
\section{Introduction}
\label{sec:intro}
Labelled datasets, even the systematically annotated ones, are noisy~\citep{Beyer_arXiv_2020_done_ImageNet}. Designing noise-robust supervised learning algorithms are, therefore, of primary importance for real-world applications. This work proposes simple loss functions based on Jensen-Shannon divergence~\citep{Lin_TIT_1991_JS_Divergence} to increase robustness of  discriminative models to label noise in a risk-minimization framework. Similar loss functions have recently been successfully adopted for test-time robustness to distributional shift~\citep{hendrycks2020augmix}. Differently, in this work, we make theoretical arguments for their robustness to label noise at training time and discuss other desirable properties such as consistency regularization in the context of prior noise-robust loss functions. Then, we show remarkable empirical efficacy on standard noisy image recognition tasks using currently most-popular machine learning models -- deep networks.

One key advantage of deep networks and its stochastic-gradient-based optimization is their resilience to label noise~\citep{Li_AIStats_2020_DeepLearningRobust}. Nevertheless, this robustness can be significantly improved via noise-robust model design. An important avenue towards noise-robust deep learning is to propose a provably-robust loss function~\citep{Ghosh_AAAI_2017_MAE}. Our work, extends that direction by proposing novel loss functions using Jensen-Shannon divergence which exhibit several theoretically-desirable properties such as consistency regularization and label smoothing in connection to prior works~\citep{Wang_ICCV_2019_Symmetric_CE,Zhang_NeurIPS_2018_Generalized_CE,Ma_ICML_2020_Normalized_Loss}. Contributions of this work are:
\begin{itemize}
\item We make a novel observation that the network's consistency is reduced for noisy labelled samples when overfitting to noise, which motivates the use of consistency regularization. 
\item We propose using Jensen-Shannon divergence~($\DJSnp$) and its multi-distribution generalization~($\DGJSnp$) as loss functions for learning with noisy labels. 
We relate $\DJSnp$ to loss functions that are based on the noise-robustness theory of \citet{Ghosh_AAAI_2017_MAE}. In particular, we prove that $\DJSnp$ generalizes CE and MAE. Furthermore, we prove that $\DGJSnp$ generalizes $\DJSnp$ by incorporating consistency regularization in a single principled loss function.
\item We provide strong, conclusive, and extensive empirical evidences for the efficacy of the proposed losses.
\end{itemize}
\vspace{-0.2cm}

\begin{figure*}
        \centering
        \begin{subfigure}[b]{0.47\textwidth} \centering \includegraphics[width=0.9\textwidth]{Figures/consistency-val-acc.pdf} \caption{Validation Accuracy} \label{fig:consistency-observation-a}
         \end{subfigure} 
         \hfill
         \begin{subfigure}[b]{0.47\textwidth} \centering \includegraphics[width=0.9\textwidth]{Figures/consistency-train-con.pdf} \caption{Consistency} \label{fig:consistency-observation-c} 
         \end{subfigure} 
         \caption{\textbf{Consistency When Overfitting to Noise.} Here we plot the evolution of the validation accuracy~(a) and a measure of consistency~(b) on the training set of CIFAR-100 for varying symmetric noise rates when learning with the cross-entropy loss. It can be seen that the consistency of the learnt function and the accuracy closely correlate. Assuming causation, suggests that enforcing consistency may help avoid fitting to noise. } \label{fig:consistency-observation}
\end{figure*}

==> 2_related_works.tex <==
\section{Extended Related Works}
\label{sup:rel-works}
% provably noise-robust loss functions
Most related to us is the avenue of handling noisy labels in deep learning via the identification and construction of \textit{noise-robust loss functions}~\citep{Ghosh_AAAI_2017_MAE,Zhang_NeurIPS_2018_Generalized_CE,Wang_ICCV_2019_Symmetric_CE,Ma_ICML_2020_Normalized_Loss}. \citet{Ghosh_AAAI_2017_MAE} derived sufficient conditions for a loss function, in empirical risk minimization (ERM) settings, to be robust to various kinds of sample-independent noise, including symmetric, symmetric non-uniform, and class-conditional. They further argued that, while CE is not a robust loss function, mean absolute error (MAE) is a loss that satisfies the robustness conditions and empirically demonstrated its effectiveness. On the other hand, \citet{Zhang_NeurIPS_2018_Generalized_CE} pointed out the challenges of training with MAE and proposed GCE which generalizes both MAE and CE losses. Tuning for this trade-off, GCE alleviates MAE's training difficulties while retaining some desirable noise-robustness properties. In a similar fashion, symmetric cross entropy (SCE)~\citep{Wang_ICCV_2019_Symmetric_CE} spans the spectrum of reverse CE as a noise-robust loss function and the standard CE. Recently, ~\citet{Ma_ICML_2020_Normalized_Loss} proposed a normalization mechanism to make arbitrary loss functions robust to noise. They, too, further combine two complementary loss functions to improve the data fitting while keeping robust to noise. The current work extends on this line of works.

% intro including less related works.
Several other directions are pursued to improve training of deep networks under noisy labelled datasets. This includes methods to \textit{identify and remove} noisy labels~\citep{Nguyen_ICLR_2020_self_ensemble,Northcutt_arXiv_2017} or \textit{identify and correct} noisy labels in a joint label-parameter optimization~\citep{ Tanaka_CVPR_2018_Joint_Optimization,Vahdat_NeurIPS_2017_CRF} and those works that design an \textit{elaborate training pipeline} for dealing with noise~\citep{Li_ICLR_2020_dividemix,Iscen_ECCV_2020,Seo_NeurIPS_2019}. In contrast to these directions, this work proposes a robust loss function based on Jensen-Shannon divergence (JS) without altering other aspects of training. In the following, we review the directions that are most related to this paper. 

% loss correction works
A close line of works to ours \textit{reweight a loss function} by a known or estimated class-conditional noise model~\citep{Natarajan_NIPS_2013}. This direction has been commonly studied for deep networks with a standard cross entropy (CE) loss~\citep{Sukhbaatar_ICLR_2015_confusion_matrix,Patrini_CVPR_2017,Han_NeurIPS_2018,Xia_NeurIPS_2019}. Assuming a class-conditional noise model, loss correction is theoretically well motivated.  

% label smoothing
A common regularization technique called \textit{label smoothing}~\citep{Szegedy_CVPR_2016_inception_label_smoothing} has been recently proposed that operates similarly to the loss correction methods. While its initial purpose was for deep networks to avoid overfitting, label smoothing has been shown to have a noticeable effect when training with noisy sets by alleviating the fit to the noise~\citep{Lukasik_ICML_2020_label_smoothing_label_noisy,Reed_arXiv_2014_bootstrapping}.

% consistency regularization
\textit{Consistency regularization} is a recently-developed technique that encourages smoothness in the learnt decision boundary by requiring minimal shifts in the learnt function when small perturbations are applied to an input sample. This technique has become increasingly common in the state-of-the-art semi-supervised learning~\citep{Miyato_PAMI_2018_VAT,Berthelot_NeurIPS_2019_mixmatch,Tarvainen_NIPS_2017_mean_teacher} and recently for dealing with noisy data~\citep{Li_ICLR_2020_dividemix}. These methods use various complicated pipelines to integrate consistency regularization in training. This work shows that a multi-distribution generalization of JS neatly incorporate such regularization.\\
\citet{hendrycks2020augmix} recently proposed AugMix, a novel data augmentation strategy in combination with a $\DGJSnp$ consistency loss to improve uncertainty estimation and robustness to image corruptions at test-time. Our work is orthogonal since we consider the task of learning under noisy labels at training time and conduct corresponding experiments. We also investigate and derive theoretical properties of the proposed loss functions. Finally, our losses are solely implemented based on $\DJSnp$/$\DGJSnp$ instead of a combination of CE and $\DGJSnp$ in case of AugMix.  However, we find it promising that $\DGJSnp$ improves robustness to both training-time label noise and test-time image corruption which further strengthens the significance of the JS-based loss functions. 

Finally, recently, \citet{Xu_NeurIPS_2019_Information_Theoretic_Mutual_Info_Loss,Wei_ICLR_2021_f_Divergence} propose loss functions with \textit{information theory} motivations. Jensen-Shannon divergence, with inherent information theoretic interpretations, naturally posits a strong connection of our work to those. Especially, the latter is a close \textit{concurrent} work that studies the general family of $f$-divergences but takes a different and complementary angle. Reconciling these two works with our study can be, indeed, a fruitful future direction which we consider beyond the scope and limitations of a single work such as ours. 






==> Figures/app_table_hp_1.tex <==
\begin{tabular}{ @{}l l c c@{}} %@{} removes space to vertical edges
 \toprule
 \multirow{2}{4em}{Dataset} & \multirow{2}{4em}{Method} & \multicolumn{1}{c}{Sym Noise} & \multicolumn{1}{c}{Asym Noise} \\ \cmidrule(lr){3-3} \cmidrule(lr){4-4}
 & & 20-80\% & 20-40\% \\
 \midrule
 \multirow{8}{5em}{CIFAR-10} & CE & [0.05, 1e-3] & [0.1, 1e-3] \\
 & BS & [0.1, 1e-3] & [0.1, 1e-3] \\
 & LS & [0.1, 5e-4] & [0.1, 1e-3] \\
 & SCE & [0.01, 5e-4] & [0.05, 1e-3] \\
 & GCE & [0.01, 5e-4] & [0.1, 1e-3] \\
 & NCE+RCE & [0.005, 1e-3] & [0.05, 1e-4] \\
 & JS & [0.01, 5e-4] & [0.1, 1e-3] \\
 & GJS & [0.1, 5e-4] & [0.1, 1e-3] \\
\midrule
%-----------------------------------------------------
%-----------------------------------------------------
 \multirow{8}{5em}{CIFAR-100} & CE & [0.4, 1e-4] & [0.2, 1e-4] \\
 & BS & [0.4, 1e-4] & [0.4, 1e-4] \\
 & LS & [0.2, 5e-5] & [0.4, 1e-4] \\
 & SCE & [0.2, 1e-4] & [0.4, 5e-5] \\
 & GCE & [0.4, 1e-5] & [0.2, 1e-4] \\
 & NCE+RCE & [0.2, 5e-5] & [0.2, 5e-5] \\
 & JS & [0.2, 1e-4] & [0.1, 1e-4] \\
 & GJS & [0.2, 5e-5] & [0.4, 1e-4] \\
 \bottomrule
\end{tabular}


==> Figures/app_table_hp_2.tex <==
\begin{tabular}{ @{}l l c c c c c c c@{}} %@{} removes space to vertical edges
 \toprule
 \multirow{2}{4em}{Dataset} & \multirow{2}{4em}{Method} & No Noise & \multicolumn{4}{c}{Sym Noise} & \multicolumn{2}{c}{Asym Noise} \\ \cmidrule(lr){3-3}\cmidrule(lr){4-7} \cmidrule(lr){8-9}
 & & 0\% & 20\% & 40\% & 60\% & 80\% & 20\% & 40\% \\
 \midrule
 \multirow{8}{5em}{CIFAR-10} %& CE & -  & - & - & - & - & - \\
 & CE & - & - & - & - & - & - & - \\
 & BS & 0.5 & 0.5 & 0.7 & 0.7 & X & 0.7 & 0.5 \\
 & LS & 0.1 & 0.5 & 0.9 & 0.7 & X & 0.1 & 0.1 \\
 & SCE & [0.2, 0.1] & [0.05, 0.1] & [0.1, 0.1] & [0.2, 1.0] & [X,X] & [0.1, 0.1] & [0.2, 1.0] \\
& GCE & 0.5 & 0.7 & 0.7 & 0.7 & X & 0.1 & 0.1 \\
 & NCE+RCE & [10, 0.1] & [10, 0.1] & [10, 0.1] & [1.0, 0.1] & [X,X] & [10, 0.1] & [1.0, 0.1] \\
  & JS & 0.1 & 0.7 & 0.7 & 0.9 & X & 0.3 & 0.3 \\
 & GJS & 0.5 & 0.3 & 0.9 & 0.1 & X & 0.3 & 0.3 \\
\midrule
%-----------------------------------------------------
%-----------------------------------------------------
 \multirow{8}{5em}{CIFAR-100} %& CE & - & - & - & - & - & - \\
 & CE & - & - & - & - & - & - \\
 & BS & 0.7 & 0.5 & 0.5 & 0.5 & 0.3 & 0.3 \\
 & LS & 0.1 & 0.7 & 0.7 & 0.7 & 0.5 & 0.7 \\
 & SCE & [0.1, 0.1] & [0.1, 0.1] & [0.1, 0.1] & [0.1, 1.0] & [0.1, 1.0] & [0.1, 1.0] \\
 & GCE & 0.5 & 0.5 & 0.5 & 0.7 & 0.7 & 0.7 \\
 & NCE+RCE & [20, 0.1] & [20, 0.1] & [20, 0.1] & [20, 0.1] & [20, 0.1] & [10, 0.1] \\
 & JS & 0.1 & 0.1 & 0.3 & 0.5 & 0.5 & 0.5 \\
 & GJS & 0.3 & 0.3 & 0.5 & 0.9 & 0.5 & 0.1 \\
 \bottomrule
\end{tabular}
